Phenomenology of WIMPy baryogenesis models

A possible connection between the abundances of baryonic and dark matter (DM) has been explored so far mostly in the context of the so-called asymmetric DM. Recently, a very different mechanism, dubbed "WIMPy baryogenesis", has been proposed to relate the baryon asymmetry to DM annihilation. The DM candidate is a weakly interacting massive particle (WIMP), and the usual WIMP scenario is slightly extended to accommodate baryogenesis, which is accomplished around the time of DM freeze-out. We construct an effective field theory that encompasses a quite general class of models which implement the WIMPy baryogenesis. Under some reasonable, simplifying assumptions, we show that a good portion of the parameter space is allowed for these models, after experimental constraints are taken into account. Bounds from the LHC require that the WIMP be heavier than 400 GeV.

==> PaxHeaders.22281/JCAP3.tex <==
30 mtime=1359125605.389683458
30 atime=1359125605.388683051
30 ctime=1359125605.390683494

